Exploring the accuracy of the equation-of-motion coupled-cluster band gap of solids

While the periodic equation-of-motion coupled-cluster (EOM-CC) method promises systematic improvement of electronic band gap calculations in solids, its practical application at the singles and doubles level (EOM-CCSD) is hindered by severe finite-size errors in feasible simulation cells. We present a hybrid approach combining EOM-CCSD with the computationally efficient $GW$ approximation to estimate thermodynamic limit band gaps for several insulators and semiconductors. Our method substantially reduces required cell sizes while maintaining accuracy. Comparisons with experimental gaps and self-consistent $GW$ calculations reveal that deviations in EOM-CCSD predictions correlate with reduced single excitation character of the excited many-electron states. Our work not only provides a computationally tractable approach to EOM-CC calculations in solids but also reveals fundamental insights into the role of single excitations in electronic-structure theory.

==> Makefile <==
figdi = $(PWD)/figures

all: main.pdf

clean:
	rm -vrf build

.PHONY: clean all

FIGURES += \
$(fig_lih) \

#LiH
FIGURES += $(figdi)/fs_conv_gw_3D_LiH_with_downsampling_all_orders.pdf
$(figdi)/fs_conv_gw_3D_LiH_with_downsampling_all_orders.pdf: ./data/scripts/LiH/gw/gw_tdl_convergence_3D_LiH_all_orders_fit.py
	cd ./data/scripts/LiH/gw/; python3 gw_tdl_convergence_3D_LiH_all_orders_fit.py
	cd ./data/scripts/LiH/gw/; mv -v fs_*pdf $(figdi)/

FIGURES += $(figdi)/eom_gw_correlation_3D_LiH_minimal_gap.pdf
$(figdi)/eom_gw_correlation_3D_LiH_minimal_gap.pdf: ./data/scripts/LiH/eom-vs-gw/eom_gw_correlation.py
	cd ./data/scripts/LiH/eom-vs-gw/; python3 eom_gw_correlation.py
	cd ./data/scripts/LiH/eom-vs-gw/; mv -v eom_*pdf $(figdi)/

FIGURES += $(figdi)/fs_conv_gw_3D_LiH_no_downsampling_all_orders_vasp_probe_charge.pdf
$(figdi)/fs_conv_gw_3D_LiH_no_downsampling_all_orders_vasp_probe_charge.pdf: ./data/scripts/LiH/gw-vasp-probe-charge/gw_tdl_convergence_3D_LiH_all_orders_fit_vasp_probe_charge.py
	cd ./data/scripts/LiH/gw-vasp-probe-charge/; python3 gw_tdl_convergence_3D_LiH_all_orders_fit_vasp_probe_charge.py
	cd ./data/scripts/LiH/gw-vasp-probe-charge/; mv -v fs_*pdf $(figdi)/

FIGURES += $(figdi)/eom_gw_correlation_3D_LiH_minimal_gap_vasp_probe_charge.pdf
$(figdi)/eom_gw_correlation_3D_LiH_minimal_gap_vasp_probe_charge.pdf: ./data/scripts/LiH/eom-vs-gw-vasp-probe-charge/eom_gw_correlation_vasp_probe_charge.py
	cd ./data/scripts/LiH/eom-vs-gw-vasp-probe-charge/; python3 eom_gw_correlation_vasp_probe_charge.py
	cd ./data/scripts/LiH/eom-vs-gw-vasp-probe-charge/; mv -v eom_*pdf $(figdi)/


#MgO
FIGURES += $(figdi)/fs_conv_gw_3D_MgO_with_downsampling_pure_cC_all_orders.pdf
$(figdi)/fs_conv_gw_3D_MgO_with_downsampling_pure_cC_all_orders.pdf: ./data/scripts/MgO/gw/pure-cC-with-ds/gw_tdl_convergence_3D_MgO_all_orders_fit.py
	cd ./data/scripts/MgO/gw/pure-cC-with-ds/; python3 gw_tdl_convergence_3D_MgO_all_orders_fit.py
	cd ./data/scripts/MgO/gw/pure-cC-with-ds/; mv -v fs_*pdf $(figdi)/

FIGURES += $(figdi)/eom_gw_correlation_3D_MgO.pdf
$(figdi)/eom_gw_correlation_3D_MgO.pdf: ./data/scripts/MgO/eom-vs-gw/pure-cC-with-ds/eom_gw_correlation.py
	cd ./data/scripts/MgO/eom-vs-gw/pure-cC-with-ds/; python3 eom_gw_correlation.py
	cd ./data/scripts/MgO/eom-vs-gw/pure-cC-with-ds/; mv -v eom_*pdf $(figdi)/



FIGURES += $(figdi)/vasp_fs_conv_gw_3D_MgO_with_ds_pure_cC_all_orders.pdf
$(figdi)/vasp_fs_conv_gw_3D_MgO_with_ds_pure_cC_all_orders.pdf: ./data/scripts/MgO/gw-vasp/gw_tdl_convergence_3D_MgO_all_orders_fit.py
	cd ./data/scripts/MgO/gw-vasp/; python3 gw_tdl_convergence_3D_MgO_all_orders_fit.py
	cd ./data/scripts/MgO/gw-vasp/; mv -v vasp_fs_*pdf $(figdi)/


FIGURES += $(figdi)/vasp_eom_gw_correlation_3D_MgO.pdf
$(figdi)/vasp_eom_gw_correlation_3D_MgO.pdf: ./data/scripts/MgO/eom-vs-gw-vasp/eom_gw_correlation.py
	cd ./data/scripts/MgO/eom-vs-gw-vasp/; python3 eom_gw_correlation.py
	cd ./data/scripts/MgO/eom-vs-gw-vasp/; mv -v vasp_eom_*pdf $(figdi)/



#FIGURES += $(figdi)/eom_gw_correlation_3D_MgO_pure_cC_no_ds_with_anisotropic.pdf
#$(figdi)/eom_gw_correlation_3D_MgO.pdf: ./data/scripts/MgO/eom-vs-gw-anisotropic/eom_gw_correlation.py
#	cd ./data/scripts/MgO/eom-vs-gw-anisotropic/; python3 eom_gw_correlation.py
#	cd ./data/scripts/MgO/eom-vs-gw-anisotropic/; mv -v eom_*pdf $(figdi)/



#BP
FIGURES += $(figdi)/fs_conv_gw_3D_BP_with_downsampling_pure_cC_all_orders_correct.pdf
$(figdi)/fs_conv_gw_3D_BP_with_downsampling_pure_cC_all_orders_correct.pdf: ./data/scripts/BP/gw/gw_tdl_convergence_3D_BP_all_orders_fit.py
	cd ./data/scripts/BP/gw/; python3 gw_tdl_convergence_3D_BP_all_orders_fit.py
	cd ./data/scripts/BP/gw/; mv -v fs_*pdf $(figdi)/

FIGURES += $(figdi)/eom_gw_correlation_3D_BP_correct.pdf
$(figdi)/eom_gw_correlation_3D_BP_correct.pdf: ./data/scripts/BP/eom-vs-gw/eom_gw_correlation.py
	cd ./data/scripts/BP/eom-vs-gw/; python3 eom_gw_correlation.py
	cd ./data/scripts/BP/eom-vs-gw/; mv -v eom_*pdf $(figdi)/

FIGURES += $(figdi)/vasp_fs_conv_gw_3D_BP_no_ds_probe_charge_ewald_all_orders.pdf
$(figdi)/vasp_fs_conv_gw_3D_BP_no_ds_probe_charge_ewald_all_orders.pdf: ./data/scripts/BP/gw-vasp/gw_tdl_convergence_3D_BP_all_orders_fit.py
	cd ./data/scripts/BP/gw-vasp/; python3 gw_tdl_convergence_3D_BP_all_orders_fit.py
	cd ./data/scripts/BP/gw-vasp/; mv -v vasp_fs_*pdf $(figdi)/

FIGURES += $(figdi)/vasp_eom_gw_correlation_3D_BP_correct.pdf
$(figdi)/vasp_eom_gw_correlation_3D_BP_correct.pdf: ./data/scripts/BP/eom-vs-gw-vasp/eom_gw_correlation.py
	cd ./data/scripts/BP/eom-vs-gw-vasp/; python3 eom_gw_correlation.py
	cd ./data/scripts/BP/eom-vs-gw-vasp/; mv -v vasp_eom_*pdf $(figdi)/


#C
FIGURES += $(figdi)/fs_conv_gw_3D_C_with_downsampling_pure_cC_all_orders.pdf
$(figdi)/fs_conv_gw_3D_C_with_downsampling_pure_cC_all_orders.pdf: ./data/scripts/C/gw/gw_tdl_convergence_3D_C_all_orders_fit.py
	cd ./data/scripts/C/gw/; python3 gw_tdl_convergence_3D_C_all_orders_fit.py
	cd ./data/scripts/C/gw/; mv -v fs_*pdf $(figdi)/

FIGURES += $(figdi)/eom_gw_correlation_3D_C.pdf
$(figdi)/eom_gw_correlation_3D_C.pdf: ./data/scripts/C/eom-vs-gw/eom_gw_correlation.py
	cd ./data/scripts/C/eom-vs-gw/; python3 eom_gw_correlation.py
	cd ./data/scripts/C/eom-vs-gw/; mv -v eom_*pdf $(figdi)/


FIGURES += $(figdi)/vasp_fs_conv_gw_3D_C_with_ds_pure_cC_all_orders.pdf
$(figdi)/vasp_fs_conv_gw_3D_C_with_ds_pure_cC_all_orders.pdf: ./data/scripts/C/gw-vasp/gw_tdl_convergence_3D_C_all_orders_fit.py
	cd ./data/scripts/C/gw-vasp/; python3 gw_tdl_convergence_3D_C_all_orders_fit.py
	cd ./data/scripts/C/gw-vasp/; mv -v vasp_fs_*pdf $(figdi)/


FIGURES += $(figdi)/vasp_eom_gw_correlation_3D_C.pdf
$(figdi)/vasp_eom_gw_correlation_3D_C.pdf: ./data/scripts/C/eom-vs-gw-vasp/eom_gw_correlation.py
	cd ./data/scripts/C/eom-vs-gw-vasp/; python3 eom_gw_correlation.py
	cd ./data/scripts/C/eom-vs-gw-vasp/; mv -v vasp_eom_*pdf $(figdi)/

#BN
FIGURES += $(figdi)/vasp_fs_conv_gw_3D_BN_with_ds_pure_cC_all_orders.pdf
$(figdi)/vasp_fs_conv_gw_3D_BN_with_ds_pure_cC_all_orders.pdf: ./data/scripts/BN/gw-vasp/gw_tdl_convergence_3D_BN_all_orders_fit.py
	cd ./data/scripts/BN/gw-vasp/; python3 gw_tdl_convergence_3D_BN_all_orders_fit.py
	cd ./data/scripts/BN/gw-vasp/; mv -v vasp_fs_*pdf $(figdi)/


FIGURES += $(figdi)/vasp_eom_gw_correlation_3D_BN.pdf
$(figdi)/vasp_eom_gw_correlation_3D_BN.pdf: ./data/scripts/BN/eom-vs-gw-vasp/eom_gw_correlation.py
	cd ./data/scripts/BN/eom-vs-gw-vasp/; python3 eom_gw_correlation.py
	cd ./data/scripts/BN/eom-vs-gw-vasp/; mv -v vasp_eom_*pdf $(figdi)/

#Si
FIGURES += $(figdi)/vasp_fs_conv_gw_3D_Si_with_ds_pure_cC_all_orders.pdf
$(figdi)/vasp_fs_conv_gw_3D_Si_with_ds_pure_cC_all_orders.pdf: ./data/scripts/Si/gw-vasp/gw_tdl_convergence_3D_Si_all_orders_fit.py
	cd ./data/scripts/Si/gw-vasp/; python3 gw_tdl_convergence_3D_Si_all_orders_fit.py
	cd ./data/scripts/Si/gw-vasp/; mv -v vasp_fs_*pdf $(figdi)/


FIGURES += $(figdi)/vasp_eom_gw_correlation_3D_Si.pdf
$(figdi)/vasp_eom_gw_correlation_3D_Si.pdf: ./data/scripts/Si/eom-vs-gw-vasp/eom_gw_correlation.py
	cd ./data/scripts/Si/eom-vs-gw-vasp/; python3 eom_gw_correlation.py
	cd ./data/scripts/Si/eom-vs-gw-vasp/; mv -v vasp_eom_*pdf $(figdi)/

#LiCl
FIGURES += $(figdi)/vasp_fs_conv_gw_3D_LiCl_with_ds_pure_cC_all_orders.pdf
$(figdi)/vasp_fs_conv_gw_3D_LiCl_with_ds_pure_cC_all_orders.pdf: ./data/scripts/LiCl/gw-vasp/gw_tdl_convergence_3D_LiCl_all_orders_fit.py
	cd ./data/scripts/LiCl/gw-vasp/; python3 gw_tdl_convergence_3D_LiCl_all_orders_fit.py
	cd ./data/scripts/LiCl/gw-vasp/; mv -v vasp_fs_*pdf $(figdi)/


FIGURES += $(figdi)/vasp_eom_gw_correlation_3D_LiCl.pdf
$(figdi)/vasp_eom_gw_correlation_3D_LiCl.pdf: ./data/scripts/LiCl/eom-vs-gw-vasp/eom_gw_correlation.py
	cd ./data/scripts/LiCl/eom-vs-gw-vasp/; python3 eom_gw_correlation.py
	cd ./data/scripts/LiCl/eom-vs-gw-vasp/; mv -v vasp_eom_*pdf $(figdi)/

#LiF
FIGURES += $(figdi)/vasp_fs_conv_gw_3D_LiF_with_ds_pure_cC_all_orders.pdf
$(figdi)/vasp_fs_conv_gw_3D_LiF_with_ds_pure_cC_all_orders.pdf: ./data/scripts/LiF/gw-vasp/gw_tdl_convergence_3D_LiF_all_orders_fit.py
	cd ./data/scripts/LiF/gw-vasp/; python3 gw_tdl_convergence_3D_LiF_all_orders_fit.py
	cd ./data/scripts/LiF/gw-vasp/; mv -v vasp_fs_*pdf $(figdi)/


FIGURES += $(figdi)/vasp_eom_gw_correlation_3D_LiF.pdf
$(figdi)/vasp_eom_gw_correlation_3D_LiF.pdf: ./data/scripts/LiF/eom-vs-gw-vasp/eom_gw_correlation.py
	cd ./data/scripts/LiF/eom-vs-gw-vasp/; python3 eom_gw_correlation.py
	cd ./data/scripts/LiF/eom-vs-gw-vasp/; mv -v vasp_eom_*pdf $(figdi)/




#H2-chain (alternating)
FIGURES += $(figdi)/eom_vs_delta_ccsd_t_h2_chain.pdf
$(figdi)/eom_vs_delta_ccsd_t_h2_chain.pdf: ./data/scripts/H2-chain/alternating/EOM-vs-Delta-CC/plot_eom_vs_delta_ccsd_t_h2_chain.py
	cd ./data/scripts/H2-chain/alternating/EOM-vs-Delta-CC/; python3 plot_eom_vs_delta_ccsd_t_h2_chain.py
	cd ./data/scripts/H2-chain/alternating/EOM-vs-Delta-CC/; mv -v eom_*pdf $(figdi)/

#r1 vs. system size
FIGURES += $(figdi)/r1_ip_vs_system_size_3D.pdf
FIGURES += $(figdi)/r1_ea_vs_system_size_3D.pdf
$(figdi)/r1_ea_vs_system_size_3D.pdf: ./data/scripts/r1_vs_system_size/plot_r1_vs_system_size_3D.py
	cd ./data/scripts/r1_vs_system_size/; python3 plot_r1_vs_system_size_3D.py
	cd ./data/scripts/r1_vs_system_size/; mv -v r1_*pdf $(figdi)/

#r1 vs gap error
FIGURES += $(figdi)/n1_vs_eom_gap_error.pdf
$(figdi)/n1_vs_eom_gap_error.pdf: ./data/scripts/n1_vs_error/n1_vs_gap_err.py
	cd ./data/scripts/n1_vs_error/; python3 n1_vs_gap_err.py
	cd ./data/scripts/n1_vs_error/; mv -v n1_*pdf $(figdi)/


#Pure eom extrapolations for LiH
#all orders (aims)
FIGURES += $(figdi)/fs_conv_eom_3D_LiH_with_downsampling_all_orders.pdf
$(figdi)/fs_conv_eom_3D_LiH_with_downsampling_all_orders.pdf: ./data/scripts/LiH/pure-eom-extrapolation/all-orders/aims/eom_tdl_convergence_3D_LiH_all_orders_fit.py
	cd ./data/scripts/LiH/pure-eom-extrapolation/all-orders/aims/; python3 eom_tdl_convergence_3D_LiH_all_orders_fit.py
	cd ./data/scripts/LiH/pure-eom-extrapolation/all-orders/aims/; mv -v fs_*pdf $(figdi)/

#all orders (vasp)
FIGURES += $(figdi)/fs_conv_eom_3D_LiH_with_downsampling_all_orders_vasp.pdf
$(figdi)/fs_conv_eom_3D_LiH_with_downsampling_all_orders_vasp.pdf: ./data/scripts/LiH/pure-eom-extrapolation/all-orders/vasp/eom_tdl_convergence_3D_LiH_all_orders_fit.py
	cd ./data/scripts/LiH/pure-eom-extrapolation/all-orders/vasp/; python3 eom_tdl_convergence_3D_LiH_all_orders_fit.py
	cd ./data/scripts/LiH/pure-eom-extrapolation/all-orders/vasp/; mv -v fs_*pdf $(figdi)/

#leading order (aims)
FIGURES += $(figdi)/fs_conv_eom_3D_LiH_with_downsampling_leading_order.pdf
$(figdi)/fs_conv_eom_3D_LiH_with_downsampling_leading_order.pdf: ./data/scripts/LiH/pure-eom-extrapolation/only-leading-order/aims/eom_tdl_convergence_3D_LiH_all_orders_fit.py
	cd ./data/scripts/LiH/pure-eom-extrapolation/only-leading-order/aims/; python3 eom_tdl_convergence_3D_LiH_all_orders_fit.py
	cd ./data/scripts/LiH/pure-eom-extrapolation/only-leading-order/aims/; mv -v fs_*pdf $(figdi)/

#leading order (vasp)
FIGURES += $(figdi)/fs_conv_eom_3D_LiH_with_downsampling_leading_order_vasp.pdf
$(figdi)/fs_conv_eom_3D_LiH_with_downsampling_leading_order_vasp.pdf: ./data/scripts/LiH/pure-eom-extrapolation/only-leading-order/vasp/eom_tdl_convergence_3D_LiH_all_orders_fit.py
	cd ./data/scripts/LiH/pure-eom-extrapolation/only-leading-order/vasp/; python3 eom_tdl_convergence_3D_LiH_all_orders_fit.py
	cd ./data/scripts/LiH/pure-eom-extrapolation/only-leading-order/vasp/; mv -v fs_*pdf $(figdi)/

#leading order (3x3x3-5x5x5) (aims)
FIGURES += $(figdi)/fs_conv_eom_3D_LiH_with_downsampling_leading_order-333-555.pdf
$(figdi)/fs_conv_eom_3D_LiH_with_downsampling_leading_order-333-555.pdf: ./data/scripts/LiH/pure-eom-extrapolation/only-leading-order-333-to-555/aims/eom_tdl_convergence_3D_LiH_all_orders_fit.py
	cd ./data/scripts/LiH/pure-eom-extrapolation/only-leading-order-333-to-555/aims/; python3 eom_tdl_convergence_3D_LiH_all_orders_fit.py
	cd ./data/scripts/LiH/pure-eom-extrapolation/only-leading-order-333-to-555/aims/; mv -v fs_*pdf $(figdi)/

#leading order (3x3x3-5x5x5) (vasp)
FIGURES += $(figdi)/fs_conv_eom_3D_LiH_with_downsampling_leading_order_vasp-333-555.pdf
$(figdi)/fs_conv_eom_3D_LiH_with_downsampling_leading_order_vasp-333-555.pdf: ./data/scripts/LiH/pure-eom-extrapolation/only-leading-order-333-to-555/vasp/eom_tdl_convergence_3D_LiH_all_orders_fit.py
	cd ./data/scripts/LiH/pure-eom-extrapolation/only-leading-order-333-to-555/vasp/; python3 eom_tdl_convergence_3D_LiH_all_orders_fit.py
	cd ./data/scripts/LiH/pure-eom-extrapolation/only-leading-order-333-to-555/vasp/; mv -v fs_*pdf $(figdi)/








supplementary.pdf: supplementary.tex supplementary.bib $(FIGURES)
	latexmk -pdf -synctex=1 -outdir=build -shell-escape supplementary.tex
	ln -sf build/supplementary.pdf



main.pdf: main.tex main.bib supplementary.pdf $(FIGURES)
	latexmk -pdf -synctex=1 -outdir=build -shell-escape main.tex
	ln -sf build/main.pdf




==> supplementaryxx.tex <==


